Elaborating Evaluation-Order Polymorphism

We classify programming languages according to evaluation order: each language fixes one evaluation order as the default, making it transparent to program in that evaluation order, and troublesome to program in the other. This paper develops a type system that is impartial with respect to evaluation order. Evaluation order is implicit in terms, and explicit in types, with by-value and by-name versions of type connectives. A form of intersection type quantifies over evaluation orders, describing code that is agnostic over (that is, polymorphic in) evaluation order. By allowing such generic code, programs can express the by-value and by-name versions of a computation without code duplication. We also formulate a type system that only has by-value connectives, plus a type that generalizes the difference between by-value and by-name connectives: it is either a suspension (by name) or a "no-op" (by value). We show a straightforward encoding of the impartial type system into the more economical one. Then we define an elaboration from the economical language to a call-by-value semantics, and prove that elaborating a well-typed source program, where evaluation order is implicit, produces a well-typed target program where evaluation order is explicit. We also prove a simulation between evaluation of the target program and reductions (either by-value or by-name) in the source program. Finally, we prove that typing, elaboration, and evaluation are faithful to the type annotations given in the source program: if the programmer only writes by-value types, no by-name reductions can occur at run time.

==> fig-assignment-impartial.tex <==

            \begin{figure}[htbp]
              \centering
                  \judgbox{\typeof{\gamma}{e}{\tau}}
                               {Source expression $e$ has source type $\tau$}
            %
                  \vspace{-3ex}
                  \begin{mathpar}
            %
            \RuleHead{\unitty}
               \Infer{\Iunitintro}
                         {}
                         {\typeof{\gamma}{\unit}{\unitty}}
               \\
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            \RuleHead{\AllSym}
            \Infer{\Iallintro}
                  {\typeof{\gamma, \alpha \type}{v}{\tau}
                  }
                  {\typeof{\gamma}{v}{\All{\alpha} \tau}}
            \and
            \Infer{\Iallelim}
                 {\typeof{\gamma}{e}{\All{\alpha} \tau}
                  \\
                  \gamma \entails \tau' \type}
                 {\typeof{\gamma}{e}{[\tau' / \alpha]\tau}}
               \\
            %
            \RuleHead{\alleosym}
            \Infer{\Ialleointro}
                  {\typeof{\gamma, \eovar \eo}{v}{\tau}
                  }
                  {\typeof{\gamma}{v}{\alleo{\eovar} \tau}}
            \and
            \Infer{\Ialleoelim}
                 {\typeof{\gamma}{e}{\alleo{\eovar} \tau}
                   \\
                   \gamma \entails \epsilon \eo}
                 {\typeof{\gamma}{e}{[\epsilon / \eovar]\tau}}
               \\
                  \Infer{\Ivar}
                        {}
                        {\typeof{\gamma, \xtypeof{x}{\tau}, \gamma'}{x}{\tau}}
                  \and
                  \Infer{\Ifix}
                        {\typeof{\gamma, \xtypeof{u}{\tau}}{e}{\tau}}
                        {\typeof{\gamma}{(\Fix{u} e)}{\tau}}
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
            %
                \\
                \RuleHead{\garr{\epsilon}}
                   \Infer{\Iarrintro}
                         {\typeof{\gamma, x:\tau_1}{e}{\tau_2}
                         }
                         {\typeof{\gamma}{(\explam{x} e)}{(\tau_1 \garr{\epsilon} \tau_2)}}
                   \and
                   \Infer{\Iarrelim}
                          {\typeof{\gamma}{e_1}{(\tau_1 \garr{\epsilon} \tau_2)}
                           \\
                           \typeof{\gamma}{e_2}{\tau_1}
                          }
                          {\typeof{\gamma}{(\expapp{e_1}{e_2})}{\tau_2}
                          }
                \\
                \RuleHead{*^\epsilon}
                      \Infer{\Iprodintro}
                             {\typeof{\gamma}{e_1}{\tau_1}
                               \\
                               \typeof{\gamma}{e_2}{\tau_2}
                              }
                              {\typeof{\gamma}{\Pair{e_1}{e_2}}{(\tau_1 *^\epsilon \tau_2)}}
                       \and
                       \Infer{\Iprodelim{k}}
                             {
                               \typeof{\gamma}
                                       {e}
                                       {(\tau_1 *^\epsilon \tau_2)}
                             }
                             {
                               \typeof{\gamma}
                                    {(\Proj{k} e)}
                                    {\tau_k}
                             }
                \\
                \RuleHead{+^\epsilon}
                   \Infer{\Isumintro{k}}
                         {\typeof{\gamma}{e}{\tau_k}
                         }
                         {\typeof{\gamma}{(\Inj{k} e)}{(\tau_1 +^\epsilon \tau_2)}}
                   \and
                   \Infer{\Isumelim}
                          {   \typeof{\gamma}{e}{(\tau_1 +^\epsilon \tau_2)}
                              \\
                              \arrayenvbl{
                                  \typeof{\gamma, x_1 : \tau_1}{e_1}{\tau}
                                  \\
                                  \typeof{\gamma, x_2 : \tau_2}{e_2}{\tau}
                              }
                          }
                          {\typeof{\gamma}{\Casesum{e}{x_1}{e_1}{x_2}{e_2}}{\tau}
                          }
                \\
                \RuleHead{\recsym{\epsilon}}
                   \Infer{\Irecintro}
                         {\typeof{\gamma}{e}{\left[(\rec{\epsilon}{\alpha}\tau)/\alpha\right]\tau}
                         }
                         {\typeof{\gamma}{e}{\rec{\epsilon}{\alpha} \tau}}
                   \and
                   \Infer{\Irecelim}
                          {   \typeof{\gamma}{e}{\rec{\epsilon}{\alpha} \tau}
                          }
                          {
                            \typeof{\gamma}{e}{[(\rec{\epsilon}{\alpha}\tau)/\alpha]\tau}
                          }
                \end{mathpar}

              \caption{Impartial type assignment system for the source language}
              \FLabel{fig:impartial-type-assignment}
            \end{figure}



==> fig-derivation-step.tex <==
\begin{figure}[htbp]
  \centering
  
  \judgbox{\D \dstep \D'}
          {Economical typing derivation $\D$ for $e$ steps to $\D'$ for $e'$}
  \begin{mathpar}
    \Infer{}
         {\Dee_0 \dstep \Dee_0'}
         {\Rallintro(\Dee_0) \dstep \Rallintro(\Dee_0)}
    \and
    \Infer{}
         {\Dee_0 \dstep \Dee_0'}
         {\Ralleointro(\Dee_0) \dstep \Ralleointro(\Dee_0)}
    \\
    \Infer{}
         {\Dee_0 \dstep \Dee_0'}
         {\Rallelim(\Dee_0) \dstep \Rallelim(\Dee_0)}
    \and
    \Infer{}
         {\Dee_0 \dstep \Dee_0'}
         {\Ralleoelim(\Dee_0) \dstep \Ralleoelim(\Dee_0)}
    \\
    \Infer{}
         {}
         {\Rsuspintro[\V](\Dee_0) \dstep \Dee_0}
    \and
    \Infer{}
         {}
         {\Rsuspelim[\V](\Dee_0) \dstep \Dee_0}
    \\
    \Infer{}
         {}
         {\Rsuspelim[\N]\big(\Ranno(\Rsuspintro[\N](\Dee_0))\big)
           \dstep
           \Ranno(\Dee_0)}
    \\
    \Infer{}
         {}
         {\Rfix(\Dee_0)
           \dstep
           \big[\Anno{(\Fix{x} e)}{S} \big/ x \big]
           \big[\Ranno(\Rfix(\Dee_0))
              \big/
              (x : S)
           \big]\Dee_0
         }
%
%
%
%
%
%
%
%
%
%
    \\
    \Infer{}
         {\Dee_0 \dstep \Dee_0'}
         {\Rsub(\Dee_0) \dstep \Rsub(\Dee_0)}
    \and
    \Infer{}
         {\Dee_0 \dstep \Dee_0'}
         {\Ranno(\Dee_0) \dstep \Ranno(\Dee_0)}
    \and
    \Infer{}
         {}
         {\Ranno\big(\Ranno(\Dee_0)\big) \dstep \Ranno(\Dee_0)}
    \\
    \Infer{}
         {\Dee_1 \dstep \Dee_1'}
         {\Rarrelim(\Dee_1, \Dee_2) \dstep \Rarrelim(\Dee_1', \Dee_2)}
    \and
    \Infer{}
         {\Dee_1 \derives \dots \xechk{e_1}{\VAL}{S}
           \\
           \Dee_2 \dstep \Dee_2'}
         {\Rarrelim(\Dee_1, \Dee_2) \dstep \Rarrelim(\Dee_1, \Dee_2')}
    \and
    \Infer{}
         {
         \Dee_2 \derives \dots \xechk{e_2}{\VAL}{S}}
         {\Rarrelim\big(\Ranno(\Dee_1 \derives \dots \Lam{x} e \dots), \Dee_2\big)
           \dstep
           \big[\Anno{e_2}{S} \big/ x \big]
           \big[\Dee_2 \big/ (x : S) \big]
           \Dee_1
         }
  \end{mathpar}
  
  \caption{Derivation-guided source reduction}
  \FLabel{fig:derivation-step}
\end{figure}


%
%
%


==> fig-diagram-talk.tex <==
\def\RfadeContingent#1#2{\ifnum\FigVersion=1
  \Rfade{#1}{#2}%
\else
  {#2}
\fi}

$\hspace{-10pt}$\begin{tikzpicture}
  [every node/.style={font=\runonfontsz{11pt}},
   auto, node distance=3cm, >=stealth, %
   descr/.style= {fill=white, inner sep=3.0pt, anchor=center}
  ]
  \node (lsrc) {%
  };
%
  \node [right of=lsrc,
          node distance=1.6cm,
          label={above:{
           $\begin{array}[t]{l@{~}l@{~}l@{~}l@{~}l}
             \varr & *^\V & +^\V & \recsym{\V}
             \\
             \narr & *^\N & +^\N & \recsym{\N}
             \\
             &~\AllSym
             &\!\RfadeContingent{1}{\alleosym}
           \end{array}$              
          }}
          ] (upperleft) {$e \synabovechk \tau\mathstrut$};
  \node [above of=upperleft, node distance=2.8cm] (upperleftabove)
          {\tabularenvl{Impartial \\ ~type system}};
  \node [above of=upperleftabove, right=0.6cm, node distance=0.75cm] (upperleftabove) {\bf Source language ($e$)};
%
  \node [right of=upperleft, node distance=3.3cm,
           label={above:{
                  \arrayenvc{
                     {\arr}
                     ~{*}
                     ~{+}
                     ~{\recsymbol}
                    \\
                    \RfadeContingent{2}{\susp{\V}}~\RfadeContingent{2}{\susp{\N}}
                    \\
                    \AllSym
                    ~~~
                      \RfadeContingent{1}{\alleosym}%
                   }
           }}
        ] (uppercentre) {$e \synabovechk S\mathstrut$};
     \node [above of=uppercentre, node distance=2.6cm]
              (uppercentreabove)
              {\tabularenvl{Economical \\ ~type system}};
     \draw [->] (upperleft)  -- node[below] {\tabularenvc{encode \\ types}} (uppercentre);
%

%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
 %

   \node[right of=uppercentre, node distance=2.0cm,
           label={above:{\textsl{er}ase types}},
   ] (uppererase) {$\er{e} : S$};

   \node[right of=uppererase, node distance=4.0cm,
           label={above:{
                  \arrayenvc{
                     {\arr}
                     ~{*}
                     ~{+}
                     ~{\recsymbol}
                    \\
                    \RfadeContingent{3}{\xU}~\text{(thunk)}
                    \\
                    \AllSym
                   }
           }}
      ] (upperright) {$M : A$};

   \node [above of=upperright, node distance=2.0cm, left=-0.9cm] (upperrightabove) {Cbv type system};

   \node [above of=upperrightabove, node distance=0.5cm, left=-1.5cm] (upperrightaboveabove) {\bf Target language ($M$)};

  \draw [right hook->] (uppererase)  -- node[below] {elaborate} (upperright);


\ifnum\FigVersion=2

  \node [below of=upperright, node distance=3.2cm] (lowerright) {$W : A$};

 \draw [|->]
      ($(upperright.south)+(-7pt,1pt)$)
            -- node[left] {%
                   \!\!\begin{tabular}{l}
                     standard cbv
                     \\
                     evaluation
                     \\
                     ($\geq 0$ steps)
                   \end{tabular}\!\!\!\!\!}
%
      ($(lowerright.north)+(-7pt,1pt)$);   


\uncover<2->{
  \node [below of=uppererase, node distance=3.2cm] (lowererase) {$e' : S$};

  \draw [right hook->, color=dRed] (lowererase)  -- node[above] {elaborate} (lowerright);

  \draw [->,
         decorate,decoration=
               {zigzag,segment length=4pt,amplitude=0.8pt,post=lineto,post length=3.5pt},
         color=dRed
      ]
      ($(uppererase.south)+(-8pt,1pt)$)
            -- node[left] {%
                   \!\!\begin{tabular}{l}
                     cbv + cbn \\ evaluation \\
                     ($\geq 0$ steps)
                   \end{tabular}\!\!\!\!}
%
      ($(lowererase.north)+(-8pt,1pt)$);   
}
   
\fi
\end{tikzpicture}

\ifnum\FigVersion=2

   If $\elab{\er e}{}{S}{M}$ and $M \step^* W$
   \uncover<2->{%
     then
   \textcolor{dRed}{$\er e \srcstep^* e'$}
   and
   \textcolor{dRed}{$\elab {e'} {} {S} {W}$}.
   }

\fi


==> fig-non-eval-context-kitchen-sink.tex <==
\begin{figure}[htbp]
  \centering
  
  \begin{mathpar}
  \RuleHead{\varr}
    \Infer{}
        {M_1 \step M_1'}
        {(M_1 \vapp M_2) \step (M_1' \vapp M_2)}
    \and
    \Infer{}
        {M_2 \step M_2'}
        {(W_1 \vapp M_2) \step (W_1 \vapp M_2')}
    \and
    \Infer{}
        {}
        {\big((\vLam{x} e) \vapp W_2\big) \step [W_2/x]e}
    \\
    \RuleHead{\narr}
    \Infer{}
        {M_1 \step M_1'}
        {(M_1 \napp M_2) \step (M_1' \napp M_2)}
    \and
    \Infer{}
        {}
        {\big((\nLam{x} e) \napp M_2\big) \step [M_2/x]e}
    \\
    \RuleHead{*}
    \Infer{}
        {M_1 \step M_1'}
        {\tpair{M_1}{M_2}
         \step
         \tpair{M_1'}{M_2}}
    \and
    \Infer{}
        {M_2 \step M_2'}
        {\tpair{W_1}{M_2}
         \step
         \tpair{W_1}{M_2'}}
    \and
    \Infer{}
        {}
        {\Proj{k}{\tpair{M_1}{M_2}}
         \step
         M_k}
    \\
    \RuleHead{+^\V}
    \Infer{}
         {M \step M'}
         {\tinj{\V}{k}{M} \step \tinj{\V}{k}{M'}}
    ~~~~~~~
    \Infer{}
         {M \step M'}
         {(\xtcase{\V}{M}{MS}) \step (\xtcase{\V}{M'}{MS})}
    \vspace{-2.0ex}
    \\
    \Infer{}
         {}
         {(\tcase{\V}{\tinj{\V}{k}{W}}{x_1}{N_1}{x_2}{N_2})
           ~\step~
           [W/x_k]N_k}
    \\
    \RuleHead{+^\N}
    \Infer{}
         {M \step M'}
         {(\xtcase{\N}{M}{MS}) \step (\xtcase{\N}{M'}{MS})}
    \vspace{-2.0ex}
    \\
    \Infer{}
         {}
         {(\tcase{\N}{\tinj{\N}{k}{W}}{x_1}{N_1}{x_2}{N_2})
           ~\step~
           [W/x_k]N_k}
  \end{mathpar}
  
  \caption{Kitchen-sink operational semantics, formulated without evaluation contexts}
  \FLabel{fig:kitchen-sink}
\end{figure}


==> fig-src-reduce.tex <==
\begin{figure}[htbp]
  \centering
  
  \judgbox{\D \dstep \D'}
          {Economical typing derivation $\D$ for $e$ steps to $\D'$ for $e'$}
  \begin{mathpar}
    \Infer{}
         {\Dee_0 \dstep \Dee_0'}
         {\Rallintro(\Dee_0) \dstep \Rallintro(\Dee_0)}
    \and
    \Infer{}
         {\Dee_0 \dstep \Dee_0'}
         {\Ralleointro(\Dee_0) \dstep \Ralleointro(\Dee_0)}
    \\
    \Infer{}
         {\Dee_0 \dstep \Dee_0'}
         {\Rallelim(\Dee_0) \dstep \Rallelim(\Dee_0)}
    \and
    \Infer{}
         {\Dee_0 \dstep \Dee_0'}
         {\Ralleoelim(\Dee_0) \dstep \Ralleoelim(\Dee_0)}
    \\
    \Infer{}
         {}
         {\Rsuspintro[\V](\Dee_0) \dstep \Dee_0}
    \and
    \Infer{}
         {}
         {\Rsuspelim[\V](\Dee_0) \dstep \Dee_0}
    \\
    \Infer{}
         {}
         {\Rsuspelim[\N]\big(\Ranno(\Rsuspintro[\N](\Dee_0))\big)
           \dstep
           \Ranno(\Dee_0)}
    \\
    \Infer{}
         {}
         {\Rfix(\Dee_0)
           \dstep
           \big[\Anno{(\Fix{u} e)}{S} \big/ u \big]
           \big[\Ranno(\Rfix(\Dee_0))
              \big/
              (u : S)
           \big]\Dee_0
         }
%
%
%
%
%
%
%
%
%
%
    \\
    \Infer{}
         {\Dee_0 \dstep \Dee_0'}
         {\Rsub(\Dee_0) \dstep \Rsub(\Dee_0)}
    \and
    \Infer{}
         {\Dee_0 \dstep \Dee_0'}
         {\Ranno(\Dee_0) \dstep \Ranno(\Dee_0)}
    \and
    \Infer{}
         {}
         {\Ranno\big(\Ranno(\Dee_0)\big) \dstep \Ranno(\Dee_0)}
    \\
    \Infer{}
         {\Dee_1 \dstep \Dee_1'}
         {\Rarrelim(\Dee_1, \Dee_2) \dstep \Rarrelim(\Dee_1', \Dee_2)}
    \and
    \Infer{}
         {\Dee_1 \derives \dots \xechk{e_1}{\VAL}{S}
           \\
           \Dee_2 \dstep \Dee_2'}
         {\Rarrelim(\Dee_1, \Dee_2) \dstep \Rarrelim(\Dee_1, \Dee_2')}
    \and
    \Infer{}
         {
         \Dee_2 \derives \dots \xechk{e_2}{\VAL}{S}}
         {\Rarrelim\big(\Ranno(\Dee_1 \derives \dots \Lam{x} e \dots), \Dee_2\big)
           \dstep
           \big[\Anno{e_2}{S} \big/ x \big]
           \big[\Dee_2 \big/ (x : S) \big]
           \Dee_1
         }
  \end{mathpar}
  
  \caption{Derivation-guided source reduction}
  \FLabel{fig:src-step}
\end{figure}


%
%
%


==> fig-subtyping.tex <==

\begin{figure}[htbp]
  \centering
  
  \begin{mathpar}
    \Infer{\SubRefl}
        {}
        {\Gamma \entails S \subtype S}
    \and
    \Infer{\SubArr}
        {
           \Gamma \entails S_2 \subtype S_1
           \\
           \Gamma \entails S_1' \subtype S_2'
        }
        {\Gamma \entails (S_1 \arr S_1') \subtype (S_2 \arr S_2')}
    \and
    \Infer{\SubProd}
        {
           \Gamma \entails S_1 \subtype S_2
           \\
           \Gamma \entails S_1' \subtype S_2'
        }
        {\Gamma \entails (S_1 * S_1') \subtype (S_2 * S_2')}
    \and
    \Infer{\SubSum}
        {
           \Gamma \entails S_1 \subtype S_2
           \\
           \Gamma \entails S_1' \subtype S_2'
        }
        {\Gamma \entails (S_1 + S_1') \subtype (S_2 + S_2')}
    \\
    \Infer{\SubRecL}
        {
           \Gamma \entails \big[(\Rec{\alpha}S_1) \big/\alpha\big]S_1 \subtype S_2
        }
        {\Gamma \entails (\Rec{\alpha} S_1) \subtype S_2}
    \and
    \Infer{\SubRecR}
        {
           \Gamma \entails S_1 \subtype \big[(\Rec{\beta}S_2) \big/\beta\big]S_2
        }
        {\Gamma \entails S_1 \subtype (\Rec{\beta} S_2)}
    \\
    \Infer{\SubAllL}
        {\Gamma \entails S' \type
          \\
          \Gamma \entails S_1 \subtype [S'/\alpha]S_2}
        {\Gamma \entails (\All{\alpha} S_1) \subtype S_2}
    \and
    \Infer{\SubAllR}
        {\Gamma, \beta \type \entails S_1 \subtype S_2}
        {\Gamma \entails S_1 \subtype (\All{\beta} S_2)}
    \\
    \Infer{\SubGateL}
        {
           \Gamma \entails S_1 \subtype S_2
        }
        {\Gamma \entails \susp{\epsilon} S_1 \subtype S_2}
    \and
    \Infer{\SubGateR}
        {
           \Gamma \entails S_1 \subtype S_2
        }
        {\Gamma \entails S_1 \subtype \susp{\epsilon} S_2}
    \\
    \Infer{\SubAlleoL}
        {\Gamma \entails \epsilon \eo
          \\
          \Gamma \entails S_1 \subtype [\epsilon/\eovar]S_2}
        {\Gamma \entails (\alleo{\eovar} S_1) \subtype S_2}
    \and
    \Infer{\SubAlleoR}
        {\Gamma, \eovar \eo \entails S_1 \subtype S_2}
        {\Gamma \entails S_1 \subtype (\alleo{\eovar} S_2)}
  \end{mathpar}
  
  \caption{Subtyping}
  \FLabel{fig:subtyping}
\end{figure}


%
%
%


==> flags.tex <==



==> kitchen-sink-elab.tex <==
\begin{figure}[htbp]
  \centering

  \judgbox{\Gamma \entails \elab{e}{S}{M}}
               {Expression $e$ translates at type $S$ to target term $M$}
              %
  \vspace{-2ex}
  \begin{mathpar}
     \Infer{\Evar}
         {}
         {\Gamma, \var{x}{S} \entails \elab{x}{S}{x}}
     \and
     \Infer{\Efix}
            {\Gamma, \var{x}{S} \entails \elab{e}{S}{M}}
            {\Gamma \entails \elab{(\Fix{x} e)}{S}{(\tfix{x} M)}}
     \and
     \Infer{\Eunitintro}
          { }
          {\Gamma \entails \elab{\unit}{\unitty}{\tunit}}

%
%
%
%
%
%
%
%
%
%
%
   \\
%
   \RuleHead{\garr{\epsilon}}
     \Infer{\Earrintro}
         {\Gamma, \var{x}{S_1} \entails
           \elab {e} {S_2} {M}
         }
         {
              \Gamma
              \entails
              \elab 
                   {(\explam {x} e)}
                   {(S_1 \garr{\epsilon} S_2)}
                   {\tlam{\epsilon}{x} M}
         }
     \and
     \Infer{\Earrelim}
          {
            \arrayenvbl{
                \Gamma \entails \elab{e_1}{(S_1 \garr{\epsilon} S_2)}{M_1}
                \\
                \Gamma \entails \elab{e_2}{S_1}{M_2}
            }
          }
          {\Gamma \entails \elab
                {(\expapp{e_1}{e_2})}
                {S_2}
                {(M_1 \app{\epsilon} M_2)
                }
          }
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
    \\
    \RuleHead{\alleosym}
    \Infer{\Ealleointro}
          {\arrayenvbl{
              \Gamma \entails \elab{v}{[\V/\eovar]S}{M_1}
              \\
              \Gamma \entails \elab{v}{[\N/\eovar]S}{M_2}
            }
          }
          {\Gamma \entails \elab{v}{\alleo{\eovar} S}{\tpair{\V}{M_1}{M_2}}
          }
   \and
   \Infer{\Ealleoelim}
       {\Gamma \entails \elab{e}{\alleo{\eovar} S}{M}}
       {
         \arrayenvbl{
              \Gamma
              \entails
              \elab{e}
                   {[\V/\eovar]S}
                   {
                     \Proj{1} M
                   }
              \\
              \Gamma
              \entails
              \elab{e}
                   {[\N/\eovar]S}
                   {
                     \Proj{2} M
                   }
         }
       }
\\
\RuleHead{\AllSym}
\Infer{\Eallintro}
      {\Gamma, \alpha \entails \elab{v}{S}{M}
      }
      {\Gamma \entails \elab{v}{\All{\alpha} S}{M}}
\and
\Infer{\Eallelim}
     {\Gamma \entails \elab{e}{\All{\alpha} S}{M}
      \\
      \Gamma \entails S'}
     {\Gamma \entails \elab{e}{[S' / \alpha]S}{M}}
   \\
    \RuleHead{+^\epsilon}
       \Infer{\Esumintro{k}}
             {\Gamma \entails \elab{e}{S_k}{M}
             }
             {\Gamma \entails \elab{(\Inj{k} e)}{S_1 +^\epsilon S_2}{\tinj{\epsilon}{k} M}}
       \and
       \Infer{\Esumelim}
              {   
                  \arrayenvbl{
                      \Gamma \entails \elab{e}{S_1 +^\epsilon S_2}{M_0} \\
                      \Gamma, x_1 : S_1 \entails \elab{e_1}{S}{M_1}
                      \\
                      \Gamma, x_2 : S_2 \entails \elab{e_2}{S}{M_2}
                  }
              }
              {\Gamma
                \entails
                \arrayenvl{
                    {\Casesum{e}{x_1}{e_1}{x_2}{e_2}}
                    :
                    {S}
                    \\
                    \elabsymbol
                    {\tcase{\epsilon}{M_0}{x_1}{M_1}{x_2}{M_2}}
                }
              }
    \\
    \RuleHead{\recsym{\epsilon}}
       \Infer{\Erecintro}
             {\Gamma \entails \elab{e}{\big[(\rec{\epsilon}{\alpha}S)/\alpha\big]S}{M}
             }
%
             {\Gamma \entails \elab{e}{\rec{\epsilon}{\alpha} S}{(\troll{\epsilon} M)}}
       \and
       \Infer{\Erecelim}
              {   \Gamma \entails \elab{e}{\rec{\epsilon}{\alpha} S}{M}
              }
%
              {
                \Gamma \entails \elab{e}{\big[(\rec{\epsilon}{\alpha}S)/\alpha\big]S}{(\tunroll{\epsilon}{M})}
              }

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
  \end{mathpar}


  \caption{Elaboration}
  \label{fig:elab}
\end{figure}



\begin{figure}[htbp]
  \centering
  In this definition, $\epsilon$ ranges over $\{\V, \N\}$, not over $\{\V, \N, \eovar\}$.

  \medskip

  \begin{tabular}[t]{rclll}
      $\tytrans{\unitty}$  &$=$&   $\unitty$
      \\
      $\tytrans{S_1 \garr{\epsilon} S_2}$  &$=$&   $\tytrans{S_1} \garr{\epsilon} \tytrans{S_2}$
      \\
      $\tytrans{S_1 +^{\epsilon} S_2}$  &$=$&   $\tytrans{S_1} +^{\epsilon} \tytrans{S_2}$
      \\
      $\tytrans{\alpha}$  &$=$&   $\alpha$
      \\
      $\tytrans{\All{\alpha} S}$  &$=$&   $\All{\alpha} \tytrans{S}$
%
      \\
      $\tytrans{\alleo{\eovar} S}$  &$=$&   $\fighi{\tytrans{[\V/\eovar]S} * \tytrans{[\N/\eovar]S}}$
      \\
      $\tytrans{\Rec{\alpha} S}$  &$=$&   $\Rec{\alpha} \tytrans{S}$
      \\[1ex]
      \\
      $\ctxtrans{\cdot}$  &$=$&   $\cdot$
      \\
      $\ctxtrans{\Gamma, \alpha \type}$  &$=$&   $\ctxtrans{\Gamma}, \alpha \type$
      \\
      $\ctxtrans{\Gamma, \xtypeof{x}{S}}$  &$=$&   $\ctxtrans{\Gamma}, \xtypeoft{x}{\tytrans{S}}$
      \\
      $\ctxtrans{\Gamma, \eovar}$  && undefined
  \end{tabular}

  \caption{Type translation}
  \FLabel{fig:tytrans}
\end{figure}


==> parameters-acm.tex <==
\def\OPTIONArxiv{0}
\def\OPTIONAppendix{0}

